Quantum Accelerator Stack: A Research Roadmap

This paper presents the definition and implementation of a quantum computer architecture to enable creating a new computational device - a quantum computer as an accelerator In this paper, we present explicitly the idea of a quantum accelerator which contains the full stack of the layers of an accelerator. Such a stack starts at the highest level describing the target application of the accelerator. Important to realise is that qubits are defined as perfect qubits, implying they do not decohere and perform good quantum gate operations. The next layer abstracts the quantum logic outlining the algorithm that is to be executed on the quantum accelerator. In our case, the logic is expressed in the universal quantum-classical hybrid computation language developed in the group, called OpenQL. We also have to start thinking about how to verify, validate and test the quantum software such that the compiler generates a correct version of the quantum circuit. The OpenQL compiler translates the program to a common assembly language, called cQASM. We need to develop a quantum operating system that manages all the hardware of the micro-architecture. The layer below the micro-architecture is responsible of the mapping and routing of the qubits on the topology such that the nearest-neighbour-constraint can be be respected. At any moment in the future when we are capable of generating multiple good qubits, the compiler can convert the cQASM to generate the eQASM, which is executable on a particular experimental device incorporating the platform-specific parameters. This way, we are able to distinguish clearly the experimental research towards better qubits, and the industrial and societal applications that need to be developed and executed on a quantum device.

==> 01-01-b2-IBM-cQASM.tex <==

\subsection{IBM-openQL combination}
this part describes the openQASM output Qiskit generates and what the cQASM is that openQL compiler generates.

\subsubsection{IBM Qiskit system}
1. programming language : Qiskit which is a open-source SDK and using Python
2. compiler: Qiskit compiler, generating openQASM, what are classical logic functions such as if then else, loops, ...
3. number of qubits: up to how many qubits can you include in your application
4. perfect qubits
5. quantum volume: achieved a volume of 64 in a 27-qubit system
6. simulator:



\subsubsection{\QX simulator and cQASM}
1. programming language : Python, C++, OpenQL
2. compiler: QASM compiler translate OpenQL to cQASM and eQASM for experimental chips
3. number of qubits: as many as we want
4. quantum volume:
5. simulator: \QX


make a table of the ibm qiskit openQASM language in terms of qubits, qubit types, amplitudes, quantum gates and describe them in terms of execution time either as wall clock time or cpu cycles, memory consumption, errors, fault tolerance(maybe),  quantum volume, 

use https://www.tablesgenerator.com

\begin{table}[]
\caption{Overview of metrics}
\label{tab:my-table}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{\# qubits} & \# Gates & \textbf{wall clock} & \textbf{CPU} & \textbf{memory} & \textbf{\begin{tabular}[c]{@{}l@{}}Q Circuit \\ Depth\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Quantum\\ Volume\end{tabular}} \\ \hline
2                  &          &                     &              &                 &                                                                     &                                                                   \\ \hline
3                  &          &                     &              &                 &                                                                     &                                                                   \\ \hline
4                  &          &                     &              &                 &                                                                     &                                                                   \\ \hline
5                  &          &                     &              &                 &                                                                     &                                                                   \\ \hline
\end{tabular}
\end{table}


==> Mapping_start.tex <==


\subsection{Scenarios: Mapping in small and large quantum systems}

The different scenarios are defined based on: i) the number of qubits, ii) the use of quantum error correction (QEC), and iii) the definition of a quantum plane architecture (e.g. communication channels). 

Before describing them, it is important to mention what kind of quantum systems we will have in the next coming years. In the near future, we will have what Preskill calls Noisy Intermediate-Scale Quantum (NISQ) systems \cite{preskill2018}. ``Intermediate-Scale'' refers to the size of quantum chips that we will have in the next coming years that will consist of 50 to a few hundreds of qubits. ``Noisy'' means that we will have imperfect control over those qubits (decoherence, faulty gates, crosstalk, etc.) and it will limit what quantum devices will be able to do.

\subsection{Mapping scenarios}
\begin{enumerate}
    
    \item \textbf{1. Small systems (tens of qubits) without QEC and without/with quantum plane architecture:} in this case we are very limited by the number of qubits, so no encoding is used. We will focus on current quantum processors that consist of $\sim$ tens of qubits. In principle, no communication infrastructure will be required. The challenge here is to identify when the definition of a quantum plane architecture pays off.   
    
    \item \textbf{2. Large systems (hundreds of qubits) without QEC and quantum plane architecture:} here we will consider hundreds of qubits and then we will define specialized areas such are communication channels.
    
    \item \textbf{3. Large systems (hundreds of qubits) with small QEC codes and quantum plane architecture:} in this scenario the main challenge will be to map the small QEC code given a specific qubits topology (connectivity) or find a qubit topology in which the small QEC code can be easily implemented. In addition it will be necessary to create an infrastructure that allows moving logical qubits in an efficient way.
    
    \item \textbf{4. Very large quantum systems (thousands of qubits) with QEC and quantum plane architecture:} here we assume a very large number of qubits (thousands) that allows to protect information using a more expensive QEC code such as surface code. \footnote{first results are shown in this paper: arXiv preprint arXiv:1805.11127, 2018.}. As in the previous case, it will be necessary to define a quantum plane architecture.
\end{enumerate}



So far we have been focusing on the first and fourth scenarios.
We are currently looking at the mapping of quantum algorithms on superconducting qubits (SC-7 and SC-17, Daniel's work) as well as on spin qubits crossbar (Alejandro's work). In addition, we have studied the fault-tolerance and implementation of logical operations for planar surface code and propose two infrastructures for the routing of planar surface code qubits (Lingling's work).

As now, and in the next coming years, we will be in the NISQ era in which chips will have not so many qubits (up to a few hundreds of qubits) and they will be noisy, we will be focusing on the first, second and third scenarios. 


\subsection {Start of the mapping analysis}

\textbf{Experiments}

During the first year, we will focus on scenarios 1 and 2, that is, small an large number of qubits, without QEC, and with or without defining a quantum plane architecture.
In addition, for small  (up to 50?) we will assume both perfect qubits, gates and measurements as well as erroneous ones. For large quantum systems (>50 qubits), we will only consider perfect qubits, gates, and measurements.

Summarizing, the experiments will be:


\begin{itemize}
    \item \textbf{No mapping, no errors} (small and large)
    \item \textbf{Mapping, no errors} (small and large)
    \item \textbf{No mapping, errors} (small)
    \item \textbf{Mapping, errors} (small)

\end{itemize}

For all experiments, as we already mentioned, we will use the following metrics: i) Quantum fidelity; ii) Probability of success; iii) number of gates; and iv) circuit depth (or latency).


\textbf{Parameter variation}
 We will vary the following parameters:
 
 \begin{itemize}
     \item \textbf{Movement operation:} SWAP, SHUTTLE, MOVE
     \item \textbf{Qubit topology:}what kind of nearest-neighbour constraint (1D array, 2D array, ring, etc.)
     \item \textbf{Quantum plane architecture:} i) communication channels (bandwidth, distribution, throughput); ii) computational areas (size, shape)
     \item \textbf{Number of qubits}: we will explore different number of qubits for both small and large systems.
     \item \textbf{Error rates:} We can take error rates from current technologies ($10^{-2}$) but also assume lower error rates ($10^{-6/7}$).
     
     
 \end{itemize}







% As we mentioned before, in the next years we will focus on scenarios 1, 2, and 3.
% In all 3 scenarios the first step will be to derive the most representative metric(s)/cost function(s) that the routing algorithm will optimize and that will be the output of the mapping model. 
% To this purpose, we will assume a specific qubit topology (i.e. a 2D array of qubits with only NN interactions) and run several algorithms (it can be just randomly generated algorithms) using different mapping models (the mapping optimize different parameters). 
% Based on those experiments, the metrics/cost functions will be defined. 









% \subsection{Scenario 1}
% In this scenario we will focus on current chips. Qubits will be noisy, the mapping model will take into account all hardware constraints (hardware dependent) and no quantum plane architecture will be defined.
% This work will be mostly developed by master students and will focus, for now, on superconducting qubits.
% As the number of qubits will be pretty low, ad-hoc mapping solutions can be developed.


% \subsection{Scenario 2 and 3}
% The only difference between these two scenarios is the use of quantum error correction. In this case, the mapping model will be hardware independent, meaning that only connectivity constraints will be taking into account (qubit topology). 
% Note that, we will maybe assume in the first phase perfect qubits but that will depend on the metrics we will use (in we want to see how the mapping affects the probability of success we meed error in the circuit). 

% After defining the right metrics/cost functions, we will run simulations in which the following parameters will be varied:

% \begin{itemize}
%     \item Number of qubits (\textcolor{red}{We will need to define a range. When does it make sense to define communication channels?})
%     \item Qubit topology (ring, 1D array, 2D array, etc)
%     \item Movement operation (SWAP, SHUTTLE, etc.)
%     \item Quantum plane architecture (number, bandwidth and distribution of communication channels, size of computational areas, etc.)
    
% \end{itemize}

% It is worth noting, that different routing strategies will be used based on the parameters mentioned above.
% Based on these experiments, we will have a reduced set of configurations that we will further study.
% To simplify the problem, we will start with scenario 2.

% \textbf{Steps}
% \begin{enumerate}
%     \item Investigate and define mapping metrics.
%     \item Definition of: i) number of qubits, ii) qubit topology, iii) movement operation, and iv) quantum plane architecture.
%     \item Based on the configurations defined in Step 2, several routing algorithms will be defined (theoretical analysis)\textcolor{red}{This is something proposed by Jose Duato in our project}.
% \end{enumerate}




% \subsection {OTP project}

% We will also have 1 PhD student working on the mapping problem for the OTP project. We will study the mapping on a Si-spin crossbar. The maximum size of the crossbar will be 1024 locations and we will take into account all hardware constraints. No QEC will be used.

% In this case, the parameters to vary will be:

% \begin{itemize}
%     \item I would use the same set of metrics, independent of what the target technology is.
%     \item Size of the crossbar
%     \item Number of data and ancilla qubits
%     \item Location of the qubits
%     \item Quantum plane architecture (if we think that is required)
% \end{itemize}

% Again, different routing strategies will need to be investigated.

% We will investigate the mapping of quantum algorithms but maybe also the mapping of small quantum error correction codes (just error syndrome measurement circuits).

\subsection{Simulation infrastructure}
 OpenQL compiler schedules the instructions (it can also include optimal initial placement) and outputs cQASM code. This code is executed on the QNoC simulator? to experiment with the different routing techniques given a specific number of qubits, qubit topology, quantum plane architecture, and movement operation.

\begin{itemize}
    \item Input: Quantum algorithm (circuit) described in OpenQL/cQASM 
    \item Mapping model: C++ code that can be implemented as a compiler pass or separate code. It should include initial placement, scheduling and routing.
    \item Output: cQASM code (after mapping) and the mapping metrics 
    \item Data base: for each combination of parameter, the mapping metrics.
\end{itemize}




\subsection{Notes}
\begin{itemize}
    \item For small number of qubits there is interest in the actual quantum result but for large number of qubits, no interest in the actual quantum result that is computed
    
    \ietm For very small number of qubits no quantum plane architecture will be defined and we can use ad-hoc routing solutions. WE will have to investigate when defining a quantum plane architecture pays off. For larger number of qubits, a quantum plane architecture will be defined and heuristics (or other approach) will be necessary for the routing algorithm.
    
    \item Next step will be to go for large number of qubits and use small QEC codes. In this case, a quantum plane architecture that allows moving logical qubits needs to de defined. The routing approach will be more or less the same.
    
    \item Noisy system: we can try different error models (depolarising, circuit, more realistic, etc. ) with different error rates. 
    
    \item QNOC simulator?
\end{itemize}








\subsection{Definitions}

\begin{itemize}
    \item Virtual qubits: qubits in the circuit/algorithm
    \item Physical quits: qubits in the chip
    \item Number of operations: number of gates in the circuit 
    \item Circuit depth: number of cycles of the algorithm after being scheduled 
    \item Circuit latency: time required to execute the circuit when time has been assigned to each cycles (It is similar to circuit depth but expressed in time instead of cycles).
    \item Quantum fidelity: it a metric that calculates the difference between the final state gotten after running the algorithm (considering errors) and the expected state (without errors). Note that this metric is calculated before measuring the qubits and then it can only be obtained by simulation, called the \QX simulator. Several runs (1000?) are required. If we consider a perfect scenario, in which qubits, gates and measurements are error free, it will be equal to 1.
    
    \item Probability of success of the algorithm: The probability of getting a correct result; that is, how many times your algorithm produces a correct result. It is calculated after measuring the qubits and it is obtained by simulation (\QX simulator) after running the algorithm several times (1000?). If the algorithm is deterministic -e.g. arithmetic operations- it will be equal to 1. If it is non-deterministic, it will be lower than one,even in a perfect scenario where qubits, gates and measurements are error free. Once errors are considered, it will go lower. 
    
    
\end{itemize}

\begin{figure}[h!]
  \centerline{
    \includegraphics[width=3in]{circuit.png}
    }
\caption{Quantum fidelity and probability of success.}
\label{circuit}
\end{figure}

\newpage

\textcolor{red}{This is what we wrote for the flagship. }


This task is focused on the design and development of a fast, scalable Quantum Network-on-Chip (QNoC) simulation tool aimed at modelling the movement and temporization of logical/physical qubits states on large-scale FT quantum circuits layouts. We assume that qubits are arranged on a 2D lattice with only nearest-neighbour interactions and that qubits are encoded using planar surface codes. The QNoC simulator will be able to model the movement primitives operating to one qubit (e.g. Pauli or Hadamard) or two qubits (CNOT or SWAP), based on the compiler passes and run-time information. The simulator will also model the layouts for physical and logical 2D qubit lattices, defined in Task \ref{task:move_and_layouts}, and the routing algorithms on these layouts, defined in Task \ref{task:routing}, guaranteeing the movement primitives completion, efficiency when selecting the communication paths, deadlock freedom and reduced contention. Based on the compiler scheduled operations, quantum instructions dependency graphs (QIDG) and the initial placement of logical/physical qubits in the 2D lattice, the QNoC simulator will trigger the communication primitives. The reason for what the QNoC simulator needs the compiler and runtime support defined in Task \ref{task:move_scheduling} is the contention that appears in the 2D lattice during movement operations and generates additional time and delays in the communication. The resources consumed by a given operation maybe required by other operations, so that it is required to look-ahead for independent movement operations that maybe triggered. The scheduling of these operations must not be static (no timestamps will be required), since the instructions sequence and operations dependencies, plus the communication dynamics (i.e. routing algorithms, contention, etc.) will determine when each operation is executed by the simulator. Finally, the simulator will provide performance metrics required to perform evaluation studies analysing the quality of the movement primitives and layouts, routing algorithms, qubit placement and scheduling of operations.
 
 \textcolor{red}{The QNoC will be initially developed as a standalone tool, but designed in such a way that it can be inserted afterwards as a compiler pass.} 
 
 
